Non intrusive method for parametric model order reduction using a bi-calibrated interpolation on the Grassmann manifold

Approximating solutions of non-linear parametrized physical problems by interpolation presents a major challenge in terms of accuracy. In fact, pointwise interpolation of such solutions is rarely efficient and leads generally to incorrect results. However, instead of using a straight forward interpolation on solutions, reduced order models can be interpolated. More particularly, Amsallem and Farhat proposed an efficient POD reduced order model interpolation technique based on differential geometry tools. This approach, named in this paper ITSGM (Interpolation On a Tangent Space of the Grassmann Manifold), allows through the passage to the tangent space of the Grassmann manifold, to approximate accurately the reduced order basis associated to a new untrained parameter. This basis is used afterwards to build the interpolated ROM describing the temporal dynamics by performing the Galerkin projection on the high fidelity model. Such Galerkin ROMs require to access to the underlying high fidelity model, leading by that to intrusive ROMs. In this paper, and contrary to the ITSGM/Galerkin approach, we propose a non-intrusive reduced order modeling method which is independent of the governing equations. This method is named through this paper Bi-CITSGM (Bi-Calibrated ITSGM). It consists first to interpolate the spatial and temporal POD sampling bases considered as representatives of points on Grassmann manifolds, by the ITSGM method. Then, the resulting bases modes are reclassified by introducing two orthogonal matrices. These calibration matrices are determined as analytical solutions of two optimization problems. Results on the flow problem past a circular cylinder where the parameter of interpolation is the Reynolds number, show that for new untrained Reynolds number values, the developed approach produces satisfyingly accurate solutions in a real computational time.

==> FIGURES/PART3/NIMR/Eigen_values/Eigen_values_pressure_sampling_points.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,704){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1342,1286){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1342,1867){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1342,2449){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1342,3030){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(1342,3612){\makebox(0,0)[r]{\strut{} 10000}}%
      \put(1342,4193){\makebox(0,0)[r]{\strut{} 100000}}%
      \put(1342,4775){\makebox(0,0)[r]{\strut{} 1e+06}}%
      \put(1474,484){\makebox(0,0){\strut{} 50}}%
      \put(2140,484){\makebox(0,0){\strut{} 100}}%
      \put(2806,484){\makebox(0,0){\strut{} 150}}%
      \put(3472,484){\makebox(0,0){\strut{} 200}}%
      \put(4139,484){\makebox(0,0){\strut{} 250}}%
      \put(4805,484){\makebox(0,0){\strut{} 300}}%
      \put(5471,484){\makebox(0,0){\strut{} 350}}%
      \put(6137,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Pressure POD eigenvalues}}}%
      \put(4138,154){\makebox(0,0){\strut{}Reynolds number}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/Eigen_values/Eigen_values_pressure_sampling_points}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/Eigen_values/Eigen_values_velocity_sampling_points.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1342,1383){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1342,2061){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1342,2740){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(1342,3418){\makebox(0,0)[r]{\strut{} 10000}}%
      \put(1342,4097){\makebox(0,0)[r]{\strut{} 100000}}%
      \put(1342,4775){\makebox(0,0)[r]{\strut{} 1e+06}}%
      \put(1474,484){\makebox(0,0){\strut{} 50}}%
      \put(2140,484){\makebox(0,0){\strut{} 100}}%
      \put(2806,484){\makebox(0,0){\strut{} 150}}%
      \put(3472,484){\makebox(0,0){\strut{} 200}}%
      \put(4139,484){\makebox(0,0){\strut{} 250}}%
      \put(4805,484){\makebox(0,0){\strut{} 300}}%
      \put(5471,484){\makebox(0,0){\strut{} 350}}%
      \put(6137,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Velocity POD eigenvalues}}}%
      \put(4138,154){\makebox(0,0){\strut{}Reynolds number}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/Eigen_values/Eigen_values_velocity_sampling_points}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/Eigen_values/LEGEND_Eigen.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3667,3509){\makebox(0,0)[r]{\strut{}mode 1}}%
      \csname LTb\endcsname%
      \put(3667,3289){\makebox(0,0)[r]{\strut{}mode 2}}%
      \csname LTb\endcsname%
      \put(3667,3069){\makebox(0,0)[r]{\strut{}mode 3}}%
      \csname LTb\endcsname%
      \put(3667,2849){\makebox(0,0)[r]{\strut{}mode 4}}%
      \csname LTb\endcsname%
      \put(3667,2629){\makebox(0,0)[r]{\strut{}mode 5}}%
      \csname LTb\endcsname%
      \put(3667,2409){\makebox(0,0)[r]{\strut{}mode 6}}%
      \csname LTb\endcsname%
      \put(3667,2189){\makebox(0,0)[r]{\strut{}mode 7}}%
      \csname LTb\endcsname%
      \put(3667,1969){\makebox(0,0)[r]{\strut{}mode 8}}%
      \csname LTb\endcsname%
      \put(3667,1749){\makebox(0,0)[r]{\strut{}mode 9}}%
      \csname LTb\endcsname%
      \put(3667,1529){\makebox(0,0)[r]{\strut{}mode 10}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/Eigen_values/LEGEND_Eigen}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/Eigen_values/LEGEND_RIC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3667,3509){\makebox(0,0)[r]{\strut{}$\nbrModes = $ 1}}%
      \csname LTb\endcsname%
      \put(3667,3289){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 2}}%
      \csname LTb\endcsname%
      \put(3667,3069){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 3}}%
      \csname LTb\endcsname%
      \put(3667,2849){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 4}}%
      \csname LTb\endcsname%
      \put(3667,2629){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 5}}%
      \csname LTb\endcsname%
      \put(3667,2409){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 6}}%
      \csname LTb\endcsname%
      \put(3667,2189){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 7}}%
      \csname LTb\endcsname%
      \put(3667,1969){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 8}}%
      \csname LTb\endcsname%
      \put(3667,1749){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 9}}%
      \csname LTb\endcsname%
      \put(3667,1529){\makebox(0,0)[r]{\strut{}$\nbrModes =  $ 10}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/Eigen_values/LEGEND_RIC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/Eigen_values/RIC_pressure_sampling_points.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 92}}%
      \put(946,1213){\makebox(0,0)[r]{\strut{} 93}}%
      \put(946,1722){\makebox(0,0)[r]{\strut{} 94}}%
      \put(946,2231){\makebox(0,0)[r]{\strut{} 95}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{} 96}}%
      \put(946,3248){\makebox(0,0)[r]{\strut{} 97}}%
      \put(946,3757){\makebox(0,0)[r]{\strut{} 98}}%
      \put(946,4266){\makebox(0,0)[r]{\strut{} 99}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1078,484){\makebox(0,0){\strut{} 50}}%
      \put(1794,484){\makebox(0,0){\strut{} 100}}%
      \put(2509,484){\makebox(0,0){\strut{} 150}}%
      \put(3225,484){\makebox(0,0){\strut{} 200}}%
      \put(3941,484){\makebox(0,0){\strut{} 250}}%
      \put(4656,484){\makebox(0,0){\strut{} 300}}%
      \put(5372,484){\makebox(0,0){\strut{} 350}}%
      \put(6087,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Ratio (\%) - pressure}}}%
      \put(3940,154){\makebox(0,0){\strut{}Reynolds number}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/Eigen_values/RIC_pressure_sampling_points}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/Eigen_values/RIC_velocity_sampling_points.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 30}}%
      \put(946,1286){\makebox(0,0)[r]{\strut{} 40}}%
      \put(946,1867){\makebox(0,0)[r]{\strut{} 50}}%
      \put(946,2449){\makebox(0,0)[r]{\strut{} 60}}%
      \put(946,3030){\makebox(0,0)[r]{\strut{} 70}}%
      \put(946,3612){\makebox(0,0)[r]{\strut{} 80}}%
      \put(946,4193){\makebox(0,0)[r]{\strut{} 90}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1078,484){\makebox(0,0){\strut{} 50}}%
      \put(1794,484){\makebox(0,0){\strut{} 100}}%
      \put(2509,484){\makebox(0,0){\strut{} 150}}%
      \put(3225,484){\makebox(0,0){\strut{} 200}}%
      \put(3941,484){\makebox(0,0){\strut{} 250}}%
      \put(4656,484){\makebox(0,0){\strut{} 300}}%
      \put(5372,484){\makebox(0,0){\strut{} 350}}%
      \put(6087,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Ratio (\%) - velocity}}}%
      \put(3940,154){\makebox(0,0){\strut{}Reynolds number}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/Eigen_values/RIC_velocity_sampling_points}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/LEGEND.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5053,2739){\makebox(0,0)[r]{\strut{}High fidelity model}}%
      \csname LTb\endcsname%
      \put(5053,2519){\makebox(0,0)[r]{\strut{}Bi-CITSGM}}%
      \csname LTb\endcsname%
      \put(5053,2299){\makebox(0,0)[r]{\strut{}ITSGM/Galerkin}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/LEGEND}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/Mean_Errors/LEGEND.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4063,2629){\makebox(0,0)[r]{\strut{}Bi-CITSGM}}%
      \csname LTb\endcsname%
      \put(4063,2409){\makebox(0,0)[r]{\strut{}ITSGM/Galerkin}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/Mean_Errors/LEGEND}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/Mean_Errors/mean_Relative_Error.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1078,484){\makebox(0,0){\strut{} 100}}%
      \put(1896,484){\makebox(0,0){\strut{} 150}}%
      \put(2714,484){\makebox(0,0){\strut{} 200}}%
      \put(3532,484){\makebox(0,0){\strut{} 250}}%
      \put(4349,484){\makebox(0,0){\strut{} 300}}%
      \put(5167,484){\makebox(0,0){\strut{} 350}}%
      \put(5985,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Mean relative error (\%)}}}%
      \put(3940,154){\makebox(0,0){\strut{}Reynolds number }}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,1097){\makebox(0,0)[r]{\strut{}Velocity}}%
      \csname LTb\endcsname%
      \put(5816,877){\makebox(0,0)[r]{\strut{}Pressure}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/Mean_Errors/mean_Relative_Error}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/Mean_Errors/mean_Relative_Error_pressure.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 0.01}}%
      \put(1078,2061){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1078,3418){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1210,484){\makebox(0,0){\strut{} 100}}%
      \put(2009,484){\makebox(0,0){\strut{} 150}}%
      \put(2808,484){\makebox(0,0){\strut{} 200}}%
      \put(3607,484){\makebox(0,0){\strut{} 250}}%
      \put(4406,484){\makebox(0,0){\strut{} 300}}%
      \put(5205,484){\makebox(0,0){\strut{} 350}}%
      \put(6004,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Mean relative error - pressure (\%)}}}%
      \put(4006,154){\makebox(0,0){\strut{}Reynolds number }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/Mean_Errors/mean_Relative_Error_pressure}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/Mean_Errors/mean_Relative_Error_velocity.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 0.01}}%
      \put(1078,2061){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1078,3418){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1210,484){\makebox(0,0){\strut{} 100}}%
      \put(2009,484){\makebox(0,0){\strut{} 150}}%
      \put(2808,484){\makebox(0,0){\strut{} 200}}%
      \put(3607,484){\makebox(0,0){\strut{} 250}}%
      \put(4406,484){\makebox(0,0){\strut{} 300}}%
      \put(5205,484){\makebox(0,0){\strut{} 350}}%
      \put(6004,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Mean relative error - velocity (\%)}}}%
      \put(4006,154){\makebox(0,0){\strut{}Reynolds number }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/Mean_Errors/mean_Relative_Error_velocity}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/LEGEND_temp_coef.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1690,2519){\makebox(0,0)[r]{\strut{}POD}}%
      \csname LTb\endcsname%
      \put(3733,2519){\makebox(0,0)[r]{\strut{}NIMR}}%
      \csname LTb\endcsname%
      \put(5776,2519){\makebox(0,0)[r]{\strut{}ITSGM/ROM}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/LEGEND_temp_coef}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{}-20}}%
      \put(814,1156){\makebox(0,0)[r]{\strut{}-15}}%
      \put(814,1609){\makebox(0,0)[r]{\strut{}-10}}%
      \put(814,2061){\makebox(0,0)[r]{\strut{}-5}}%
      \put(814,2513){\makebox(0,0)[r]{\strut{} 0}}%
      \put(814,2966){\makebox(0,0)[r]{\strut{} 5}}%
      \put(814,3418){\makebox(0,0)[r]{\strut{} 10}}%
      \put(814,3870){\makebox(0,0)[r]{\strut{} 15}}%
      \put(814,4323){\makebox(0,0)[r]{\strut{} 20}}%
      \put(814,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(946,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1478,484){\makebox(0,0){\strut{} 7}}%
      \put(2011,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2543,484){\makebox(0,0){\strut{} 8}}%
      \put(3076,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3608,484){\makebox(0,0){\strut{} 9}}%
      \put(4141,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4673,484){\makebox(0,0){\strut{} 10}}%
      \put(5206,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5738,484){\makebox(0,0){\strut{} 11}}%
      \put(6271,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{p}{1} (t)$}}%
      \put(3874,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_0}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}-2}}%
      \put(946,1213){\makebox(0,0)[r]{\strut{}-1.5}}%
      \put(946,1722){\makebox(0,0)[r]{\strut{}-1}}%
      \put(946,2231){\makebox(0,0)[r]{\strut{}-0.5}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,3248){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(946,3757){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,4266){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1078,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1598,484){\makebox(0,0){\strut{} 7}}%
      \put(2119,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2639,484){\makebox(0,0){\strut{} 8}}%
      \put(3160,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3680,484){\makebox(0,0){\strut{} 9}}%
      \put(4201,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4721,484){\makebox(0,0){\strut{} 10}}%
      \put(5242,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5762,484){\makebox(0,0){\strut{} 11}}%
      \put(6283,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{p}{2} (t)$}}%
      \put(3940,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}-1.4}}%
      \put(946,1156){\makebox(0,0)[r]{\strut{}-1.2}}%
      \put(946,1609){\makebox(0,0)[r]{\strut{}-1}}%
      \put(946,2061){\makebox(0,0)[r]{\strut{}-0.8}}%
      \put(946,2513){\makebox(0,0)[r]{\strut{}-0.6}}%
      \put(946,2966){\makebox(0,0)[r]{\strut{}-0.4}}%
      \put(946,3418){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(946,3870){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,4323){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1078,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1598,484){\makebox(0,0){\strut{} 7}}%
      \put(2119,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2639,484){\makebox(0,0){\strut{} 8}}%
      \put(3160,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3680,484){\makebox(0,0){\strut{} 9}}%
      \put(4201,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4721,484){\makebox(0,0){\strut{} 10}}%
      \put(5242,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5762,484){\makebox(0,0){\strut{} 11}}%
      \put(6283,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{p}{3} (t)$}}%
      \put(3940,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}-1}}%
      \put(946,1111){\makebox(0,0)[r]{\strut{}-0.8}}%
      \put(946,1518){\makebox(0,0)[r]{\strut{}-0.6}}%
      \put(946,1925){\makebox(0,0)[r]{\strut{}-0.4}}%
      \put(946,2332){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,3147){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(946,3554){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(946,3961){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(946,4368){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1598,484){\makebox(0,0){\strut{} 7}}%
      \put(2119,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2639,484){\makebox(0,0){\strut{} 8}}%
      \put(3160,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3680,484){\makebox(0,0){\strut{} 9}}%
      \put(4201,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4721,484){\makebox(0,0){\strut{} 10}}%
      \put(5242,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5762,484){\makebox(0,0){\strut{} 11}}%
      \put(6283,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{p}{4} (t)$}}%
      \put(3940,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}-1}}%
      \put(946,1111){\makebox(0,0)[r]{\strut{}-0.8}}%
      \put(946,1518){\makebox(0,0)[r]{\strut{}-0.6}}%
      \put(946,1925){\makebox(0,0)[r]{\strut{}-0.4}}%
      \put(946,2332){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,3147){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(946,3554){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(946,3961){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(946,4368){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1598,484){\makebox(0,0){\strut{} 7}}%
      \put(2119,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2639,484){\makebox(0,0){\strut{} 8}}%
      \put(3160,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3680,484){\makebox(0,0){\strut{} 9}}%
      \put(4201,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4721,484){\makebox(0,0){\strut{} 10}}%
      \put(5242,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5762,484){\makebox(0,0){\strut{} 11}}%
      \put(6283,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{p}{5} (t)$}}%
      \put(3940,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(1078,1213){\makebox(0,0)[r]{\strut{}-0.15}}%
      \put(1078,1722){\makebox(0,0)[r]{\strut{}-0.1}}%
      \put(1078,2231){\makebox(0,0)[r]{\strut{}-0.05}}%
      \put(1078,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1078,3248){\makebox(0,0)[r]{\strut{} 0.05}}%
      \put(1078,3757){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1078,4266){\makebox(0,0)[r]{\strut{} 0.15}}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1210,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1718,484){\makebox(0,0){\strut{} 7}}%
      \put(2227,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2735,484){\makebox(0,0){\strut{} 8}}%
      \put(3244,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3752,484){\makebox(0,0){\strut{} 9}}%
      \put(4261,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4769,484){\makebox(0,0){\strut{} 10}}%
      \put(5278,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5786,484){\makebox(0,0){\strut{} 11}}%
      \put(6295,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{p}{6} (t)$}}%
      \put(4006,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_5}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_6.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(1078,1213){\makebox(0,0)[r]{\strut{}-0.15}}%
      \put(1078,1722){\makebox(0,0)[r]{\strut{}-0.1}}%
      \put(1078,2231){\makebox(0,0)[r]{\strut{}-0.05}}%
      \put(1078,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1078,3248){\makebox(0,0)[r]{\strut{} 0.05}}%
      \put(1078,3757){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1078,4266){\makebox(0,0)[r]{\strut{} 0.15}}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1210,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1718,484){\makebox(0,0){\strut{} 7}}%
      \put(2227,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2735,484){\makebox(0,0){\strut{} 8}}%
      \put(3244,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3752,484){\makebox(0,0){\strut{} 9}}%
      \put(4261,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4769,484){\makebox(0,0){\strut{} 10}}%
      \put(5278,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5786,484){\makebox(0,0){\strut{} 11}}%
      \put(6295,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{p}{7} (t)$}}%
      \put(4006,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeP_6}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{}-30}}%
      \put(814,1383){\makebox(0,0)[r]{\strut{}-20}}%
      \put(814,2061){\makebox(0,0)[r]{\strut{}-10}}%
      \put(814,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(814,3418){\makebox(0,0)[r]{\strut{} 10}}%
      \put(814,4097){\makebox(0,0)[r]{\strut{} 20}}%
      \put(814,4775){\makebox(0,0)[r]{\strut{} 30}}%
      \put(946,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1478,484){\makebox(0,0){\strut{} 7}}%
      \put(2011,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2543,484){\makebox(0,0){\strut{} 8}}%
      \put(3076,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3608,484){\makebox(0,0){\strut{} 9}}%
      \put(4141,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4673,484){\makebox(0,0){\strut{} 10}}%
      \put(5206,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5738,484){\makebox(0,0){\strut{} 11}}%
      \put(6271,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{u}{1} (t)$}}%
      \put(3874,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_0}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{}-25}}%
      \put(814,1111){\makebox(0,0)[r]{\strut{}-20}}%
      \put(814,1518){\makebox(0,0)[r]{\strut{}-15}}%
      \put(814,1925){\makebox(0,0)[r]{\strut{}-10}}%
      \put(814,2332){\makebox(0,0)[r]{\strut{}-5}}%
      \put(814,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(814,3147){\makebox(0,0)[r]{\strut{} 5}}%
      \put(814,3554){\makebox(0,0)[r]{\strut{} 10}}%
      \put(814,3961){\makebox(0,0)[r]{\strut{} 15}}%
      \put(814,4368){\makebox(0,0)[r]{\strut{} 20}}%
      \put(814,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(946,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1478,484){\makebox(0,0){\strut{} 7}}%
      \put(2011,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2543,484){\makebox(0,0){\strut{} 8}}%
      \put(3076,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3608,484){\makebox(0,0){\strut{} 9}}%
      \put(4141,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4673,484){\makebox(0,0){\strut{} 10}}%
      \put(5206,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5738,484){\makebox(0,0){\strut{} 11}}%
      \put(6271,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{u}{2} (t)$}}%
      \put(3874,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}-5}}%
      \put(682,1111){\makebox(0,0)[r]{\strut{}-4}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{}-3}}%
      \put(682,1925){\makebox(0,0)[r]{\strut{}-2}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{}-1}}%
      \put(682,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 1}}%
      \put(682,3554){\makebox(0,0)[r]{\strut{} 2}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 3}}%
      \put(682,4368){\makebox(0,0)[r]{\strut{} 4}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 5}}%
      \put(814,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1358,484){\makebox(0,0){\strut{} 7}}%
      \put(1903,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2447,484){\makebox(0,0){\strut{} 8}}%
      \put(2992,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3536,484){\makebox(0,0){\strut{} 9}}%
      \put(4081,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4625,484){\makebox(0,0){\strut{} 10}}%
      \put(5170,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5714,484){\makebox(0,0){\strut{} 11}}%
      \put(6259,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{u}{3} (t)$}}%
      \put(3808,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}-5}}%
      \put(682,1111){\makebox(0,0)[r]{\strut{}-4}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{}-3}}%
      \put(682,1925){\makebox(0,0)[r]{\strut{}-2}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{}-1}}%
      \put(682,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 1}}%
      \put(682,3554){\makebox(0,0)[r]{\strut{} 2}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 3}}%
      \put(682,4368){\makebox(0,0)[r]{\strut{} 4}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 5}}%
      \put(814,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1358,484){\makebox(0,0){\strut{} 7}}%
      \put(1903,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2447,484){\makebox(0,0){\strut{} 8}}%
      \put(2992,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3536,484){\makebox(0,0){\strut{} 9}}%
      \put(4081,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4625,484){\makebox(0,0){\strut{} 10}}%
      \put(5170,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5714,484){\makebox(0,0){\strut{} 11}}%
      \put(6259,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{u}{4} (t)$}}%
      \put(3808,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}-4}}%
      \put(682,1383){\makebox(0,0)[r]{\strut{}-3}}%
      \put(682,2061){\makebox(0,0)[r]{\strut{}-2}}%
      \put(682,2740){\makebox(0,0)[r]{\strut{}-1}}%
      \put(682,3418){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,4097){\makebox(0,0)[r]{\strut{} 1}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 2}}%
      \put(814,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1358,484){\makebox(0,0){\strut{} 7}}%
      \put(1903,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2447,484){\makebox(0,0){\strut{} 8}}%
      \put(2992,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3536,484){\makebox(0,0){\strut{} 9}}%
      \put(4081,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4625,484){\makebox(0,0){\strut{} 10}}%
      \put(5170,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5714,484){\makebox(0,0){\strut{} 11}}%
      \put(6259,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{u}{5} (t)$}}%
      \put(3808,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}-2}}%
      \put(946,1213){\makebox(0,0)[r]{\strut{}-1.5}}%
      \put(946,1722){\makebox(0,0)[r]{\strut{}-1}}%
      \put(946,2231){\makebox(0,0)[r]{\strut{}-0.5}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,3248){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(946,3757){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,4266){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1078,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1598,484){\makebox(0,0){\strut{} 7}}%
      \put(2119,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2639,484){\makebox(0,0){\strut{} 8}}%
      \put(3160,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3680,484){\makebox(0,0){\strut{} 9}}%
      \put(4201,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4721,484){\makebox(0,0){\strut{} 10}}%
      \put(5242,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5762,484){\makebox(0,0){\strut{} 11}}%
      \put(6283,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{u}{6} (t)$}}%
      \put(3940,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_5}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_6.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}-2}}%
      \put(946,1213){\makebox(0,0)[r]{\strut{}-1.5}}%
      \put(946,1722){\makebox(0,0)[r]{\strut{}-1}}%
      \put(946,2231){\makebox(0,0)[r]{\strut{}-0.5}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,3248){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(946,3757){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,4266){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1078,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1598,484){\makebox(0,0){\strut{} 7}}%
      \put(2119,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2639,484){\makebox(0,0){\strut{} 8}}%
      \put(3160,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3680,484){\makebox(0,0){\strut{} 9}}%
      \put(4201,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4721,484){\makebox(0,0){\strut{} 10}}%
      \put(5242,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5762,484){\makebox(0,0){\strut{} 11}}%
      \put(6283,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\makebox(0,0){\strut{}$\Tmode{u}{7} (t)$}}%
      \put(3940,154){\makebox(0,0){\strut{} Time }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/Temporal_modes/TmodeU_6}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/aerodynamics_coeffs/CD.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 1.24}}%
      \put(1078,1383){\makebox(0,0)[r]{\strut{} 1.26}}%
      \put(1078,2061){\makebox(0,0)[r]{\strut{} 1.28}}%
      \put(1078,2740){\makebox(0,0)[r]{\strut{} 1.3}}%
      \put(1078,3418){\makebox(0,0)[r]{\strut{} 1.32}}%
      \put(1078,4097){\makebox(0,0)[r]{\strut{} 1.34}}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{} 1.36}}%
      \put(1210,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1718,484){\makebox(0,0){\strut{} 7}}%
      \put(2227,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2735,484){\makebox(0,0){\strut{} 8}}%
      \put(3244,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3752,484){\makebox(0,0){\strut{} 9}}%
      \put(4261,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4769,484){\makebox(0,0){\strut{} 10}}%
      \put(5278,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5786,484){\makebox(0,0){\strut{} 11}}%
      \put(6295,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}$C_D$}}}%
      \put(4006,154){\makebox(0,0){\strut{} Temps }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/aerodynamics_coeffs/CD}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/aerodynamics_coeffs/CL.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}-0.8}}%
      \put(946,1213){\makebox(0,0)[r]{\strut{}-0.6}}%
      \put(946,1722){\makebox(0,0)[r]{\strut{}-0.4}}%
      \put(946,2231){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(946,2740){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,3248){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(946,3757){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(946,4266){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(1078,484){\makebox(0,0){\strut{} 6.5}}%
      \put(1598,484){\makebox(0,0){\strut{} 7}}%
      \put(2119,484){\makebox(0,0){\strut{} 7.5}}%
      \put(2639,484){\makebox(0,0){\strut{} 8}}%
      \put(3160,484){\makebox(0,0){\strut{} 8.5}}%
      \put(3680,484){\makebox(0,0){\strut{} 9}}%
      \put(4201,484){\makebox(0,0){\strut{} 9.5}}%
      \put(4721,484){\makebox(0,0){\strut{} 10}}%
      \put(5242,484){\makebox(0,0){\strut{} 10.5}}%
      \put(5762,484){\makebox(0,0){\strut{} 11}}%
      \put(6283,484){\makebox(0,0){\strut{} 11.5}}%
      \put(6803,484){\makebox(0,0){\strut{} 12}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}$C_L$}}}%
      \put(3940,154){\makebox(0,0){\strut{} Temps }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/RESULTS_ITSGM_NIROM/RE195/aerodynamics_coeffs/CL}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/CD_mean.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{} 1.295}}%
      \put(1210,1213){\makebox(0,0)[r]{\strut{} 1.3}}%
      \put(1210,1722){\makebox(0,0)[r]{\strut{} 1.305}}%
      \put(1210,2231){\makebox(0,0)[r]{\strut{} 1.31}}%
      \put(1210,2739){\makebox(0,0)[r]{\strut{} 1.315}}%
      \put(1210,3248){\makebox(0,0)[r]{\strut{} 1.32}}%
      \put(1210,3757){\makebox(0,0)[r]{\strut{} 1.325}}%
      \put(1210,4266){\makebox(0,0)[r]{\strut{} 1.33}}%
      \put(1210,4775){\makebox(0,0)[r]{\strut{} 1.335}}%
      \put(1342,484){\makebox(0,0){\strut{} 100}}%
      \put(2122,484){\makebox(0,0){\strut{} 150}}%
      \put(2902,484){\makebox(0,0){\strut{} 200}}%
      \put(3682,484){\makebox(0,0){\strut{} 250}}%
      \put(4463,484){\makebox(0,0){\strut{} 300}}%
      \put(5243,484){\makebox(0,0){\strut{} 350}}%
      \put(6023,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}$\overline{C}_D$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Reynolds number }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/CD_mean}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/CL_max.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(946,1286){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(946,1867){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(946,2449){\makebox(0,0)[r]{\strut{} 0.7}}%
      \put(946,3030){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(946,3612){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(946,4193){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(1078,484){\makebox(0,0){\strut{} 100}}%
      \put(1896,484){\makebox(0,0){\strut{} 150}}%
      \put(2714,484){\makebox(0,0){\strut{} 200}}%
      \put(3532,484){\makebox(0,0){\strut{} 250}}%
      \put(4349,484){\makebox(0,0){\strut{} 300}}%
      \put(5167,484){\makebox(0,0){\strut{} 350}}%
      \put(5985,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}$C_{L,\max}$}}}%
      \put(3940,154){\makebox(0,0){\strut{}Reynolds number }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/CL_max}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/Crms.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 0.25}}%
      \put(1078,1111){\makebox(0,0)[r]{\strut{} 0.3}}%
      \put(1078,1518){\makebox(0,0)[r]{\strut{} 0.35}}%
      \put(1078,1925){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1078,2332){\makebox(0,0)[r]{\strut{} 0.45}}%
      \put(1078,2739){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1078,3147){\makebox(0,0)[r]{\strut{} 0.55}}%
      \put(1078,3554){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(1078,3961){\makebox(0,0)[r]{\strut{} 0.65}}%
      \put(1078,4368){\makebox(0,0)[r]{\strut{} 0.7}}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{} 0.75}}%
      \put(1210,484){\makebox(0,0){\strut{} 100}}%
      \put(2009,484){\makebox(0,0){\strut{} 150}}%
      \put(2808,484){\makebox(0,0){\strut{} 200}}%
      \put(3607,484){\makebox(0,0){\strut{} 250}}%
      \put(4406,484){\makebox(0,0){\strut{} 300}}%
      \put(5205,484){\makebox(0,0){\strut{} 350}}%
      \put(6004,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}$C_{L,rms}$}}}%
      \put(4006,154){\makebox(0,0){\strut{}Reynolds number }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/Crms}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/LEGEND.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4393,2739){\makebox(0,0)[r]{\strut{}High fidelity model}}%
      \csname LTb\endcsname%
      \put(4393,2519){\makebox(0,0)[r]{\strut{}Bi-CITSGM}}%
      \csname LTb\endcsname%
      \put(4393,2299){\makebox(0,0)[r]{\strut{}ITSGM/Galerkin}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/LEGEND}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/mean_Relative_Error_pressure.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,1364){\makebox(0,0)[r]{\strut{} 0.001}}%
      \put(1210,2217){\makebox(0,0)[r]{\strut{} 0.01}}%
      \put(1210,3070){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1210,3922){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1210,4775){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1342,1144){\makebox(0,0){\strut{} 100}}%
      \put(2122,1144){\makebox(0,0){\strut{} 150}}%
      \put(2902,1144){\makebox(0,0){\strut{} 200}}%
      \put(3682,1144){\makebox(0,0){\strut{} 250}}%
      \put(4463,1144){\makebox(0,0){\strut{} 300}}%
      \put(5243,1144){\makebox(0,0){\strut{} 350}}%
      \put(6023,1144){\makebox(0,0){\strut{} 400}}%
      \put(6803,1144){\makebox(0,0){\strut{} 450}}%
      \put(176,3069){\rotatebox{-270}{\makebox(0,0){\strut{}Mean relative error - pressure (\%)}}}%
      \put(4072,814){\makebox(0,0){\strut{}Nombre de Reynolds }}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3905,393){\makebox(0,0)[r]{\strut{}POD}}%
      \csname LTb\endcsname%
      \put(3905,173){\makebox(0,0)[r]{\strut{}POD/Galerkin}}%
      \csname LTb\endcsname%
      \put(5948,393){\makebox(0,0)[r]{\strut{}Bi-CITSGM}}%
      \csname LTb\endcsname%
      \put(5948,173){\makebox(0,0)[r]{\strut{}ITSGM/Galerkin}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/mean_Relative_Error_pressure}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/mean_Relative_Error_velocity.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,1364){\makebox(0,0)[r]{\strut{} 0.001}}%
      \put(1210,2217){\makebox(0,0)[r]{\strut{} 0.01}}%
      \put(1210,3070){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1210,3922){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1210,4775){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1342,1144){\makebox(0,0){\strut{} 100}}%
      \put(2122,1144){\makebox(0,0){\strut{} 150}}%
      \put(2902,1144){\makebox(0,0){\strut{} 200}}%
      \put(3682,1144){\makebox(0,0){\strut{} 250}}%
      \put(4463,1144){\makebox(0,0){\strut{} 300}}%
      \put(5243,1144){\makebox(0,0){\strut{} 350}}%
      \put(6023,1144){\makebox(0,0){\strut{} 400}}%
      \put(6803,1144){\makebox(0,0){\strut{} 450}}%
      \put(176,3069){\rotatebox{-270}{\makebox(0,0){\strut{}Mean relative error - velocity (\%)}}}%
      \put(4072,814){\makebox(0,0){\strut{}Nombre de Reynolds }}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3905,393){\makebox(0,0)[r]{\strut{}POD}}%
      \csname LTb\endcsname%
      \put(3905,173){\makebox(0,0)[r]{\strut{}POD/Galerkin}}%
      \csname LTb\endcsname%
      \put(5948,393){\makebox(0,0)[r]{\strut{}Bi-CITSGM}}%
      \csname LTb\endcsname%
      \put(5948,173){\makebox(0,0)[r]{\strut{}ITSGM/Galekin}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/mean_Relative_Error_velocity}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/strouhal.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{enhanced}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{} 0.155}}%
      \put(1210,1213){\makebox(0,0)[r]{\strut{} 0.16}}%
      \put(1210,1722){\makebox(0,0)[r]{\strut{} 0.165}}%
      \put(1210,2231){\makebox(0,0)[r]{\strut{} 0.17}}%
      \put(1210,2740){\makebox(0,0)[r]{\strut{} 0.175}}%
      \put(1210,3248){\makebox(0,0)[r]{\strut{} 0.18}}%
      \put(1210,3757){\makebox(0,0)[r]{\strut{} 0.185}}%
      \put(1210,4266){\makebox(0,0)[r]{\strut{} 0.19}}%
      \put(1210,4775){\makebox(0,0)[r]{\strut{} 0.195}}%
      \put(1342,484){\makebox(0,0){\strut{} 100}}%
      \put(2122,484){\makebox(0,0){\strut{} 150}}%
      \put(2902,484){\makebox(0,0){\strut{} 200}}%
      \put(3682,484){\makebox(0,0){\strut{} 250}}%
      \put(4463,484){\makebox(0,0){\strut{} 300}}%
      \put(5243,484){\makebox(0,0){\strut{} 350}}%
      \put(6023,484){\makebox(0,0){\strut{} 400}}%
      \put(6803,484){\makebox(0,0){\strut{} 450}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Strouhal number}}}%
      \put(4072,154){\makebox(0,0){\strut{}Reynolds number}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./FIGURES/PART3/NIMR/mean_aerodynamics_coeffs/strouhal}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Tex_Files/NIMR.tex <==
Consider the truncated SVD decomposition
\begin{equation*}
\SnapMatrix_i \approx \Mat{U}_{i} \Mat{\Sigma}_i \Mat{V}_{i}^T, \hspace*{0.3cm} i=1,\cdots,\nbrBases
\end{equation*}
where $\Mat{U}_i \in \mbb{R}^{\dimVecorsSnap\times \nbrModes}$ and $\Mat{V}_i \in \mbb{R}^{\nbrSnap \times \nbrModes}$ are the spatial and temporal bases such that
$$\Mat{U}_i^T \Mat{U}_i = \Mat{V}_i^T \Mat{V}_i = I_{\nbrModes}$$
and $\Sigma_i = diag\left(\sigma_{i,1}, \sigma_{i,2}, \cdots,\sigma_{i,\nbrModes}\right)$, is the diagonal matrix verifying
$$\sigma_{i,j} = \sqrt{\lambda_j(\SnapMatrix_i^T\SnapMatrix_i)} \geq \sigma_{i,j+1}, \txt{ pour }  j = 1,\cdots, \nbrModes-1$$



The first step of the Bi-CITSGM method is to approximate the matrix of singular values $\widetilde{\Mat{\Sigma}} = \Mat{\Sigma}(\widetilde{\ctrlvar})$. This can be done by simply applying a usual interpolation method, such as Spline, RBF, or Lagrange interpolations. Next, by using the ITSGM method, the subspaces $[\Mat{U}_i]$ for $i=1,dots,\nbrBases$ (resp. $[\Mat{V}_i]$) are interpolated to obtain the approximeted subspace $[\widetilde{\Mat{U}}]$ (resp. $[\widetilde{\Mat{U}}]$) for the new untrained parameter $\widetilde{\ctrlvar}$. Since $\widetilde{\Mat{U}}$ and $\widetilde{\Mat{V}}$ are only two possible representative bases of the interpolated subspaces $[\widetilde{\Mat{U}}]$ and $[\widetilde{\Mat{U}}]$, the expression of the approximated snapshots matrix $\widetilde{\SnapMatrix}$ must be expressed as follows
\begin{equation*}
\widetilde{\SnapMatrix} = \widetilde{\Mat{U}} \Mat{Q}_x \widetilde{\Sigma} \Mat{Q}_t^T \widetilde{\Mat{V}}^T
\end{equation*}
where $\Mat{Q}_x,\Mat{Q}_t \in \left[\mcal{O}(q)\right]^2$ play the role of calibration matrices. These two matrices are of a big significance in the expression of $\widetilde{\SnapMatrix}$, in fact, there good choice insures the adequate combination of column vectors of $\widetilde{\Mat{U}}$ and $\widetilde{\Mat{V}}$ which fits well with the classification of the interpolated singular values matrix $\widetilde{\Sigma}$.
%
%
The question of finding the best calibration matrices $\Mat{Q}_x$ and $\Mat{Q}_t$ is a delicate task. This paper is dedicated to propose a practical approach to solve this problem. The steps of determining $\MatCalib{K}$ and $\MatCalib{Q}$ are the same, thus, the methodology is described only for the finding of the spatial calibration matrix $\MatCalib{K}$. The same steps applies to determine the temporal calibration matrix $\MatCalib{Q}$.
First of all, the modes signs of sampling spatial and temporal bases must be adjusted with respect to a reference basis. This reference basis denoted $\Mat{U}_{k_0}$ is determined such that 
$$ k_0 = \underset{i=1,\dots,\nbrModes}{\txt{\textbf{argmin}}} \ \ \distGrass{\widetilde{\Mat{U}}}{\Mat{U}_i} $$
Once $\Mat{U}_{k_0}$ is known, using the 2-norm, the signs adjustment is performed by algorithm \ref{Alg:ajust_signs_NIMR}.
\\
\begin{algorithm}[H]
 \SetAlgoLined
\For{$k=1,\dots,\nbrBases$}{
\For{$j=1,\dots,\nbrModes$ \textbf{and} $j\neq j_0$}{
	{\small If $ || \Mat{U}_{j_0}^j - \Mat{U}_k^j ||_2 > || \widetilde{\Mat{U}}^j + \Mat{U}_k^j ||_2$ $ \Rightarrow$ multiply the $j^{\txt{th}}$ mode $\Mat{U}_k^j$ of the basis $\Mat{U}_k$ by $-1$.}	
	}	
}
\caption{Spatial bases modes signs adjustment.}
\label{Alg:ajust_signs_NIMR}
\end{algorithm}
Now that the spatial bases are signs adjusted, the calibration matrix $\Mat{Q}_x$ is looked after as the solution of the constrained minimization problem
%
%
%
\begin{equation}\label{Eq : minimization_problems_NIMR}
\underset{\Mat{\delta K}\in \mcal{O}(q)}{\txt{min}} \ \ \somme{i}{1}{\nbrBases} \omega_i  || \widetilde{\Mat{U}}  \Mat{\delta K} - \Mat{U}_{i}||_F^2
\end{equation}
where $||\cdot||_F$ is the Frobenius norm and the NIMR spatial weights $\omega_i$ are such that $\somme{i}{1}{\nbrBases} \omega_i = 1$ and given for $m>1$ as follows
\begin{equation}\label{NIMR_spatial_weights}
\omega_i = \myfrac{\distGrass{\widetilde{\Mat{U}}}{\Mat{U}_{i}}^{-m}}{\somme{k}{1}{\nbrBases} \distGrass{\widetilde{\Mat{U}}}{\Mat{U}_{k}}^{-m}} 
\end{equation}
\begin{proposition}
Given the eigendecomposition of the matrix
$$\somme{j}{1}{\nbrBases}  \somme{i}{1}{\nbrBases} \omega_i \omega_j\Mat{U}_{i}^T\widetilde{\Mat{U}} \widetilde{\Mat{U}}^T \Mat{U}_{j} = \Mat{P} \Mat{\lambda} \Mat{P}^T $$
The minimization problem \eqref{Eq : minimization_problems_NIMR} admits a unique solution given by
\begin{equation*}
\Mat{Q}_x = \widetilde{\Mat{U}}^T \left( \somme{i}{1}{\nbrBases} \omega_i\Mat{U}_{i} \right) \Mat{P} \Mat{\lambda}^{- \frac{1}{2}} \Mat{P}^T
\end{equation*}
\end{proposition}
\begin{proof}
The Lagrange function associated to the constrained minimization problem \eqref{Eq : minimization_problems_NIMR} is given by
\begin{align*}
\mcal{L}(\Mat{Q}_x,\Mat{R}) 
&=  \somme{i}{1}{\nbrBases} \omega_i || \widetilde{\Mat{U}} \Mat{ K} - \Mat{U}_{i}||_F^2 + \txt{Trace}\left(  \Mat{R}(\Mat{Q}_x^T\Mat{Q}_x - I_q) \right)
\\
&=  \somme{i}{1}{\nbrBases} \omega_i || \widetilde{\Mat{U}} \Mat{ K}||_F^2  - 2 \somme{i}{1}{\nbrBases} \omega_i \left< \widetilde{\Mat{U}} \Mat{ K},\Mat{U}_{i}\right>_F +  \somme{i}{1}{\nbrBases} \omega_i || \Mat{U}_{i}||_F^2 + \txt{Trace}\left(  \Mat{R}(\Mat{Q}_x^T\Mat{Q}_x - I_q) \right)
\end{align*}
where $\Mat{R}$ is a symmetric matrix referred to as the "Lagrange multiplier". Considering the fact that $\somme{i}{1}{\nbrBases} \omega_i = 1$, the Lagrange function simplifies to
\begin{align*}
\mcal{L}(\Mat{Q}_x,\Mat{R}) 
&=  \txt{Trace}\left( \Mat{ K}^T \underbrace{\widetilde{\Mat{U}}^T \widetilde{\Mat{U}}}_{I_{\nbrModes}} \Mat{ K} \right)  - 2 \somme{i}{1}{\nbrBases} \omega_i \txt{Trace}\left( \Mat{U}_{i}^T \widetilde{\Mat{U}} \Mat{ K} \right) 
\\
& \hspace*{1.5cm} +  \somme{i}{1}{\nbrBases} \omega_i \txt{Trace}\left( \underbrace{\Mat{U}_{i}^T \Mat{U}_{i}}_{I_{\nbrModes}} \right) + \txt{Trace}\left(  \Mat{R}(\Mat{Q}_x^T\Mat{Q}_x - I_q) \right)
\\
&=  \txt{Trace}\left( \Mat{ K}^T  \Mat{ K} \right)  - 2 \somme{i}{1}{\nbrBases} \omega_i \txt{Trace}\left( \Mat{U}_{i}^T \widetilde{\Mat{U}} \Mat{ K} \right) + \txt{Trace}\left(  \Mat{R}(\Mat{Q}_x^T\Mat{Q}_x - I_q) \right) +  \nbrModes
\end{align*}
Using the following differentiation identities
\begin{align*}
\myfrac{d}{d \Mat{B}} Trace(\Mat{A} \Mat{B}^T\Mat{B}) &= \Mat{B} (\Mat{A} + \Mat{A}^T) \\
\myfrac{d}{d \Mat{B}} Trace(\Mat{A} \Mat{B})&= \Mat{A}^T
\end{align*}
the differential of $\mcal{L}$ with respect to $\Mat{\delta K}$ writes
\begin{equation}\label{Eq : differentielle Lag wrt K}
\deriveepartielle{\mcal{L}}{\Mat{Q}_x}(\Mat{Q}_x,\Mat{R}) = 2\Mat{ K} - 2 \somme{i}{1}{\nbrBases} \omega_i \widetilde{\Mat{U}}^T\Mat{U}_{i} + 2 \Mat{Q}_x\Mat{R}
\end{equation}
When $\deriveepartielle{\mcal{L}}{\Mat{Q}_x}(\Mat{Q}_x,\Mat{R}) $ vanishes, $\Mat{Q}_x$ is a stationary point characterized by the following equation
\begin{equation}\label{Eq: gradient_Lag_NIMR}
\Mat{Q}_x \left(  I_q + \Mat{R}\right)  = \somme{i}{1}{\nbrBases} \omega_i \widetilde{\Mat{U}}^T \Mat{U}_{i} 
\end{equation}
It follows that
\begin{equation}
\left(  I_q + \Mat{R}\right)^T  \Mat{Q}_x^T  \Mat{Q}_x \left(  I_q + \Mat{R}\right)  = \somme{i}{1}{\nbrBases} \somme{j}{1}{\nbrBases}  \omega_i \omega_j \Mat{U}_{j}^T\widetilde{\Mat{U}} \widetilde{\Mat{U}}^T \Mat{U}_{i} 
\end{equation}
Given that $\Mat{Q}_x$ is orthonormal and that $\Mat{R}$ is symmetric, we can write
\begin{equation}
I_q + \Mat{R}  = \left( \underbrace{\somme{j}{1}{\nbrBases}  \somme{i}{1}{\nbrBases} \omega_i \omega_j\Mat{U}_{i}^T\widetilde{\Mat{U}} \widetilde{\Mat{U}}^T \Mat{U}_{j} }_{\Mat{M}}  \right)^{\frac{1}{2}}
\end{equation}
$\Mat{M}$ is a symmetric positive matrix, thus $M^{\frac{1}{2}}$ exists and can be calculated via the eigendecomposition of the matrix $\Mat{M}$ as follows 
\begin{equation}
\Mat{M}^{\frac{1}{2}} = \Mat{P} \Mat{\lambda}^{\frac{1}{2}} \Mat{P}^T
\end{equation}
where $\Mat{\lambda}$ eigenvalues matrix of $\Mat{M}$ and $\Mat{P}$ the associated eigenvectors matrix. 
The matrix $I_q + \Mat{R}$ is then expressed as follows 
\begin{equation}\label{Eq: Expression I_q+R}
I_q + \Mat{R}  = \Mat{P} \Mat{\lambda}^{\frac{1}{2}} \Mat{P}^T
\end{equation}
Finally, by plugging the expression of $I_q + \Mat{R}$ into the equation \eqref{Eq: gradient_Lag_NIMR}, the spatial calibration matrix $\Mat{Q}_x$ is expressed as follows
\begin{equation*}
\Mat{Q}_x = \widetilde{\Mat{U}}^T \left( \somme{i}{1}{\nbrBases} \omega_i\Mat{U}_{i} \right) \Mat{P} \Mat{\lambda}^{- \frac{1}{2}} \Mat{P}^T
\end{equation*}
\end{proof}

In the same fashion, let $\kappa_i$ be the NIMR temporal weights given by 
\begin{equation}\label{NIMR_temporal_weights}
\kappa_i = \myfrac{\distGrass{\widetilde{\Mat{V}}}{\Mat{V}_{i}}^{-m}}{\somme{k}{1}{\nbrBases} \distGrass{\widetilde{\Mat{V}}}{\Mat{V}_{k}}^{-l}}
\end{equation}
such that $l\geq 1$ and $\somme{i}{1}{\nbrBases} \kappa_i = 1$ . It can be shown that the temporal calibration matrix $\Mat{Q}_t$ is expressed as follows
\begin{equation*}
\Mat{Q}_t =  \widetilde{\Mat{V}}^T \left( \somme{i}{1}{\nbrBases} \kappa_i\Mat{V}_{i} \right)  \Mat{H} \Mat{\eta}^{- \frac{1}{2}} \Mat{H}^T
\end{equation*}
where the matrices $\Mat{H}$ and $\Mat{\eta}$ satisfy the following eigendecomposition
\begin{equation*}
\somme{j}{1}{\nbrBases} \somme{i}{1}{\nbrBases}  \kappa_i \kappa_j\Mat{V}_{i}^T\widetilde{\Mat{V}} \widetilde{\Mat{V}}^T \Mat{V}_{j} = \Mat{H} \Mat{\eta} \Mat{H}^T
\end{equation*}
The different steps of the NIMR method are resumed in algorithm \ref{alg:NIMR}.
\\
\begin{algorithm}[H]
\SetAlgoLined
%\underline{\textbf{\textit{Étape offline}:}}
\KwOffline{}
For $i=1,\dots,\nbrBases$, approximate the snapshots matrix $\SnapMatrix_i$ by the truncated SVD decomposition of order $\nbrModes$, that is
$$\SnapMatrix_i \approx \Mat{U}_{i} \Mat{\Sigma}_i \Mat{V}_{i}^T$$
\\
\KwOnline{}
Interpolate singular values matrices $\Mat{\Sigma}_{i}, \cdots, \Mat{\Sigma}_{i}$ and construct the matrix $\widetilde{\Mat{\Sigma}}$ associated to the untrained parameter $\widetilde{\ctrlvar}$.
\\
interpolate $[\Mat{U}_{i}]$ and $[\Mat{V}_{i}]$, $i=1,\dots,\nbrBases$ by using the ITSGM method and obtain $\widetilde{\Mat{U}}$ and $\widetilde{\Mat{V}}$ a spatial and temporal basis for the untrained parameter $\widetilde{\ctrlvar}$.
\\
Find the reference bases $\Mat{U}_{k_0}$ and $\Mat{U}_{l_0}$ and adjust signs of the sampling bases by algorithm \ref{Alg:ajust_signs_NIMR}.
\\
Calculate NIMR weights $\omega_j$ and $\kappa_j$ using equations \eqref{NIMR_spatial_weights} and \eqref{NIMR_temporal_weights}.
\\
Obtain $\Mat{\lambda}$, $\Mat{P}$, $\Mat{\eta}$ and $\Mat{H}$ by performing the eigendecompositions
$$\somme{j}{1}{\nbrBases}\somme{i}{1}{\nbrBases} \omega_i \omega_j\Mat{U}_{i}^T\widetilde{\Mat{U}} \widetilde{\Mat{U}}^T \Mat{U}_{j}=\Mat{P} \Mat{\lambda}  \Mat{P}^T
\hspace*{1cm}
\somme{j}{1}{\nbrBases}\somme{i}{1}{\nbrBases}  \kappa_i \kappa_j\Mat{V}_{i}^T\widetilde{\Mat{V}} \widetilde{\Mat{V}}^T \Mat{V}_{j} = \Mat{H} \Mat{\eta} \Mat{H}^T$$
\\
Calculate calibration matrices $\Mat{Q}_x$ et $\Mat{Q}_t$ as follows
$$\Mat{Q}_x =  \widetilde{\Mat{U}}^T \left( \somme{i}{1}{\nbrBases} \omega_i\Mat{U}_{i} \right) \Mat{P} \Mat{\lambda}^{- \frac{1}{2}} \Mat{P}^T
\hspace*{1cm}
\Mat{Q}_t =  \widetilde{\Mat{V}}^T \left( \somme{i}{1}{\nbrBases} \kappa_i\Mat{V}_{i} \right)  \Mat{H} \Mat{\eta}^{- \frac{1}{2}} \Mat{H}^T$$
\\
Reconstruction of the interpolated snapshots matrix
$$\widetilde{\SnapMatrix} = \widetilde{\Mat{U}} \Mat{Q}_x \widetilde{\Sigma} \Mat{Q}_t^T \widetilde{\Mat{V}}^T$$
\caption{Algorithme NIMR.}
\label{alg:NIMR}
\end{algorithm} 


==> Tex_Files/NIMR_new_temp.tex <==
Let's assume that for $i\in \{1,\dots,\nbrBases \}$, $\SnapMatrix_i$ is approximated in the low dimensional subspace $span(\Sbase{i})$ obtained by the POD method \footnote{Here, the POD basis can be chosen to be optimal with respect to any inner product, namely, $L^2$ or $H^1$ inner product.}. that means that $\SnapMatrix_i$ can be written as
\begin{equation}
\SnapMatrix_i \approx \Sbase{i} \Tbase{i}^T
\end{equation}
where $\Sbase{i}\in \mbb{R}^{\dimVecorsSnap\times \nbrModes}$ and $\Tbase{i} \in \mbb{R}^{\nbrSnap \times \nbrModes}$ verify
\begin{equation}
\integOmega{\Smode{i}{j} \Smode{i}{k}} = \delta_{jk} \hspace*{0.5cm} \txt{and} \hspace*{0.5cm} \Tmode{i}{j}^T \Tmode{i}{k} = \tau_{jk} \delta_{ij}
\end{equation}
Let $\Mat{U}_i$ the basis obtained by applying the Gram Schmidt Orthonormalization to $\Sbase{i}$, it is possible to recover the SVD form of $\SnapMatrix_i$ as follows
\begin{equation*}
\SnapMatrix_i \approx \Mat{U}_{i} \Mat{\Sigma}_i \Mat{V}_{i}^T
\end{equation*}
where $\Mat{U}_{i} = \Sbase{i}\Tbase{i}^T\Mat{V}_{i} \Mat{\Sigma}_i^{-\frac{1}{2}}$ such that $\Mat{U}_i^T \Mat{U}_i = I_{\nbrModes}$ and $\Mat{\Sigma}_i$ and $\Mat{V}_{i}$ verify the following eigendecomposition
\begin{equation}
\Tbase{i}\Sbase{i}^T\Sbase{i} \Tbase{i}^T \Mat{V}_{i} =  \Mat{\Sigma}_i \Mat{V}_{i}
\end{equation}
%Consider the truncated SVD decomposition
%\begin{equation*}
%\SnapMatrix_i \approx \Mat{U}_{i} \Mat{\Sigma}_i \Mat{V}_{i}^T, \hspace*{0.3cm} i=1,\cdots,\nbrBases
%\end{equation*}
%where $\Mat{U}_i \in \mbb{R}^{\dimVecorsSnap\times \nbrModes}$ and $\Mat{V}_i \in \mbb{R}^{\nbrSnap \times \nbrModes}$ are the spatial and temporal bases such that
%$$\Mat{U}_i^T \Mat{U}_i = \Mat{V}_i^T \Mat{V}_i = I_{\nbrModes}$$
%and $\Sigma_i = diag\left(\sigma_{i,1}, \sigma_{i,2}, \cdots,\sigma_{i,\nbrModes}\right)$, is the diagonal matrix verifying
%$$\sigma_{i,j} = \sqrt{\lambda_j(\SnapMatrix_i^T\SnapMatrix_i)} \geq \sigma_{i,j+1}, \txt{ pour }  j = 1,\cdots, \nbrModes-1$$
%
%
%
The first step of the $\nonintrusivemethod$ method is to approximate the matrix of singular values $\widetilde{\Mat{\Sigma}} = \Mat{\Sigma}(\widetilde{\ctrlvar})$. This can be done by simply applying a usual interpolation method, such as Spline, RBF, or Lagrange interpolations. Next, by using the ITSGM method, the subspaces $[\Mat{U}_i]$ for $i=1,dots,\nbrBases$ (resp. $[\Mat{V}_i]$) are interpolated to obtain the approximeted subspace $[\widetilde{\Mat{U}}]$ (resp. $[\widetilde{\Mat{U}}]$) for the new untrained parameter $\widetilde{\ctrlvar}$. Since $\widetilde{\Mat{U}}$ and $\widetilde{\Mat{V}}$ are only two possible representative bases of the interpolated subspaces $[\widetilde{\Mat{U}}]$ and $[\widetilde{\Mat{U}}]$, the expression of the approximated snapshots matrix $\widetilde{\SnapMatrix}$ must be expressed as follows
\begin{equation*}
\widetilde{\SnapMatrix} = \widetilde{\Mat{U}} \Mat{K} \widetilde{\Sigma} \Mat{Q}^T \widetilde{\Mat{V}}^T
\end{equation*}
where $\Mat{K},\Mat{Q} \in \left[\mcal{O}(q)\right]^2$ play the role of calibration matrices. These two matrices are of a big significance in the expression of $\widetilde{\SnapMatrix}$, in fact, there good choice insures the adequate combination of column vectors of $\widetilde{\Mat{U}}$ and $\widetilde{\Mat{V}}$ which fits well with the classification of the interpolated singular values matrix $\widetilde{\Sigma}$.
%
%
The question of finding the best calibration matrices $\Mat{K}$ and $\Mat{Q}$ is a delicate task. This paper is dedicated to propose a practical approach to solve this problem. The steps of determining $\MatCalib{K}$ and $\MatCalib{Q}$ are the same, thus, the methodology is described only for the finding of the spatial calibration matrix $\MatCalib{K}$. The same steps applies to determine the temporal calibration matrix $\MatCalib{Q}$.
First of all, the modes signs of sampling spatial and temporal bases must be adjusted with respect to a reference basis. This reference basis denoted $\Mat{U}_{k_0}$ is determined such that 
$$ k_0 = \underset{i=1,\dots,\nbrModes}{\txt{\textbf{argmin}}} \ \ \distGrass{\widetilde{\Mat{U}}}{\Mat{U}_i} $$
Once $\Mat{U}_{k_0}$ is known, using the 2-norm, the signs adjustment is performed by algorithm \ref{Alg:ajust_signs_NIMR}.
\\
\begin{algorithm}[H]
 \SetAlgoLined
\For{$k=1,\dots,\nbrBases$}{
\For{$j=1,\dots,\nbrModes$ \textbf{and} $j\neq j_0$}{
	{\small If $ || \Mat{U}_{j_0}^j - \Mat{U}_k^j ||_2 > || \widetilde{\Mat{U}}^j + \Mat{U}_k^j ||_2$ $ \Rightarrow$ multiply the $j^{\txt{th}}$ mode $\Mat{U}_k^j$ of the basis $\Mat{U}_k$ by $-1$.}	
	}	
}
\caption{Spatial bases modes signs adjustment.}
\label{Alg:ajust_signs_NIMR}
\end{algorithm}
Now that the spatial bases are signs adjusted, the calibration matrix $\Mat{K}$ is looked after as the solution of the constrained minimization problem
%
%
%
\begin{equation}\label{Eq : minimization_problems_NIMR}
\underset{\Mat{\delta K}\in \mcal{O}(q)}{\txt{min}} \ \ \somme{i}{1}{\nbrBases} \omega_i  || \widetilde{\Mat{U}}  \Mat{\delta K} - \Mat{U}_{i}||_F^2
\end{equation}
where $||\cdot||_F$ is the Frobenius norm and the NIMR spatial weights $\omega_i$ are such that $\somme{i}{1}{\nbrBases} \omega_i = 1$ and given for $m>1$ as follows
\begin{equation}\label{NIMR_spatial_weights}
\omega_i = \myfrac{\distGrass{\widetilde{\Mat{U}}}{\Mat{U}_{i}}^{-m}}{\somme{k}{1}{\nbrBases} \distGrass{\widetilde{\Mat{U}}}{\Mat{U}_{k}}^{-m}} 
\end{equation}
%To solve the 
%
%
%
%\begin{proposition}
%Given the eigendecomposition of the matrix
%$$\somme{j}{1}{\nbrBases}  \somme{i}{1}{\nbrBases} \omega_i \omega_j\Mat{U}_{i}^T\widetilde{\Mat{U}} \widetilde{\Mat{U}}^T \Mat{U}_{j} = \Mat{P} \Mat{\lambda} \Mat{P}^T $$
%The minimization problem \eqref{Eq : minimization_problems_NIMR} admits a unique solution given by
%\begin{equation*}
%\Mat{K} = \widetilde{\Mat{U}}^T \left( \somme{i}{1}{\nbrBases} \omega_i\Mat{U}_{i} \right) \Mat{P} \Mat{\lambda}^{- \frac{1}{2}} \Mat{P}^T
%\end{equation*}
%\end{proposition}
%\begin{proof}
The Lagrange function associated to the constrained minimization problem \eqref{Eq : minimization_problems_NIMR} is written as follows
\begin{align*}
\mcal{L}(\Mat{K},\Mat{R}) 
&=  \somme{i}{1}{\nbrBases} \omega_i || \widetilde{\Mat{U}} \Mat{ K} - \Mat{U}_{i}||_F^2 + \txt{Trace}\left(  \Mat{R}(\Mat{K}^T\Mat{K} - I_q) \right)
\end{align*}
where $\Mat{R}$ is a symmetric matrix referred to as the "Lagrange multiplier". Considering the fact that $\somme{i}{1}{\nbrBases} \omega_i = 1$, the Lagrange function simplifies to
\begin{align*}
%\mcal{L}(\Mat{K},\Mat{R}) 
%&=  \somme{i}{1}{\nbrBases} \omega_i || \widetilde{\Mat{U}} \Mat{ K}||_F^2  - 2 \somme{i}{1}{\nbrBases} \omega_i \left< \widetilde{\Mat{U}} \Mat{ K},\Mat{U}_{i}\right>_F +  \somme{i}{1}{\nbrBases} \omega_i || \Mat{U}_{i}||_F^2 + \txt{Trace}\left(  \Mat{R}(\Mat{K}^T\Mat{K} - I_q) \right)
%\\
%&=  
%\txt{Trace}\left( \Mat{ K}^T \underbrace{\widetilde{\Mat{U}}^T \widetilde{\Mat{U}}}_{I_{\nbrModes}} \Mat{ K} \right)  - 2 \somme{i}{1}{\nbrBases} \omega_i \txt{Trace}\left( \Mat{U}_{i}^T \widetilde{\Mat{U}} \Mat{ K} \right) 
%\\
%& \hspace*{1.5cm} +  \somme{i}{1}{\nbrBases} \omega_i \txt{Trace}\left( \underbrace{\Mat{U}_{i}^T \Mat{U}_{i}}_{I_{\nbrModes}} \right) + \txt{Trace}\left(  \Mat{R}(\Mat{K}^T\Mat{K} - I_q) \right)
%\\
\mcal{L}(\Mat{K},\Mat{R}) =  \txt{Trace}\left( \Mat{ K}^T  \Mat{ K} \right)  - 2 \somme{i}{1}{\nbrBases} \omega_i \txt{Trace}\left( \Mat{U}_{i}^T \widetilde{\Mat{U}} \Mat{ K} \right) + \txt{Trace}\left(  \Mat{R}(\Mat{K}^T\Mat{K} - I_q) \right) +  \nbrModes
\end{align*}
Using the following differentiation identities
\begin{align*}
\myfrac{d}{d \Mat{B}} Trace(\Mat{A} \Mat{B}^T\Mat{B}) &= \Mat{B} (\Mat{A} + \Mat{A}^T) \\
\myfrac{d}{d \Mat{B}} Trace(\Mat{A} \Mat{B})&= \Mat{A}^T
\end{align*}
The differential of $\mcal{L}$ with respect to $\Mat{K}$ gives
\begin{equation}\label{Eq : differentielle Lag wrt K}
\deriveepartielle{\mcal{L}}{\Mat{K}}(\Mat{K},\Mat{R}) = 2\Mat{ K} - 2 \widetilde{\Mat{U}}^T \somme{i}{1}{\nbrBases} \omega_i \Mat{U}_{i} + 2 \Mat{K}\Mat{R}
\end{equation}
When $\deriveepartielle{\mcal{L}}{\Mat{K}}(\Mat{K},\Mat{R}) $ vanishes, $\Mat{K}$ is a stationary point characterized by the following equation
\begin{equation}\label{Eq: gradient_Lag_NIMR}
\Mat{K} \left(  I_q + \Mat{R}\right)  = \widetilde{\Mat{U}}^T \somme{i}{1}{\nbrBases} \omega_i  \Mat{U}_{i} 
\end{equation}
Consider the SVD decomposition of the matrix 
\begin{equation}\label{Eq: SVD K(I+R)}
%\widetilde{\Mat{U}}^T \somme{i}{1}{\nbrBases} \omega_i \Mat{U}_{i} = \Mat{\xi} \Mat{\Theta} \Mat{\eta}^T
\Mat{K} \left(  I_q + \Mat{R}\right)  = \Mat{\xi} \Mat{\Theta} \Mat{\eta}^T
\end{equation}
It follows that
\begin{equation}
\left(  I_q + \Mat{R}\right)^T  \Mat{K}^T  \Mat{K} \left(  I_q + \Mat{R}\right)  = \Mat{\eta} \Mat{\Theta}^2 \Mat{\eta}^T
\end{equation}
Given that $\Mat{K}$ is orthonormal and that $\Mat{R}$ is symmetric, we can write
\begin{equation}
I_q + \Mat{R}  = \Mat{\eta} \Mat{\Theta} \Mat{\eta}^T
\end{equation}
By plugging the expression of $I_q + \Mat{R}$ into the equation \eqref{Eq: SVD K(I+R)}, the spatial calibration matrix $\Mat{K}$ is expressed as follows
\begin{equation*}
\Mat{K} =  \Mat{\xi} \Mat{\eta}^T
\end{equation*}
%\end{proof}
In the same fashion, consider the NIMR temporal weights given by 
\begin{equation}\label{NIMR_temporal_weights}
\kappa_i = \myfrac{\distGrass{\widetilde{\Mat{V}}}{\Mat{V}_{i}}^{-l}}{\somme{k}{1}{\nbrBases} \distGrass{\widetilde{\Mat{V}}}{\Mat{V}_{k}}^{-l}}
\end{equation}
such that $l\geq 1$ and $\somme{i}{1}{\nbrBases} \kappa_i = 1$. If $\Mat{\zeta} \Mat{\delta} \Mat{\gamma}^T$ is the SVD decomposition of $\widetilde{\Mat{V}}^T \somme{i}{1}{\nbrBases} \kappa_i  \Mat{V}_{i} $, it can be shown that the temporal calibration matrix $\Mat{Q}$ is expressed as follows
\begin{equation*}
\Mat{Q} =  \Mat{\zeta} \Mat{\gamma}^T
\end{equation*}
\begin{remark}
%If the matrix $\widetilde{\Mat{U}}^T \somme{i}{1}{\nbrBases} \omega_i \Mat{U}_{i}$ (respectively $\widetilde{\Mat{V}}^T \somme{i}{1}{\nbrBases} \kappa_i  \Mat{V}_{i} $) is singular, which means that $\Mat{\Theta}$ (respectively $\delta$) contains at least one zero singular value, it
If the matrix $\Mat{A} = \widetilde{\Mat{U}}^T \somme{i}{1}{\nbrBases} \omega_i \Mat{U}_{i}$ is singular, we can use SVD to approximate its inverse called pseudo-inverse with the following matrix  
\begin{equation}
\Mat{A}^{-1} \approx \Mat{A}^+ = \Mat{\eta} \Mat{\Theta}^+ \Mat{\xi}^T
\end{equation}
where for a small threshold $\varepsilon>0$, the matrix $\Mat{\Theta}^+$ is given by 
\begin{equation}
\Mat{\Theta}^+ = 
\begin{cases}
1/\theta_i \hspace*{0.2cm}&\txt{if } \theta_i>\varepsilon 
\\
0 \hspace*{0.2cm}&\txt{otherwise} 
\end{cases}
\end{equation}
In this case, the spatial calibration matrix is approximated as follows
\begin{equation}
\Mat{K} \approx  \Mat{\xi} \Mat{I}_{_{\Mat{K}}}^+ \Mat{\eta}^T
\end{equation}
where 
\begin{equation}
\Mat{I}_{_{\Mat{K}}}^+ = 
\begin{cases}
1 \hspace*{0.2cm}&\txt{if } \theta_i>\varepsilon 
\\
0 \hspace*{0.2cm}&\txt{otherwise} 
\end{cases}
\end{equation}
%such that $\Mat{I}^+ = \Mat{\Theta}\Mat{\Theta}^+$.
The same remark applies to approximate the temporal calibration matrix and we have
\begin{equation}
\Mat{Q} \approx  \Mat{\zeta} \Mat{I}_{_{\Mat{Q}}}^+ \Mat{\gamma}^T
\end{equation}
where 
\begin{equation}
\Mat{I}_{_{\Mat{Q}}}^+ = 
\begin{cases}
1 \hspace*{0.2cm}&\txt{if } \delta_i>\varepsilon 
\\
0 \hspace*{0.2cm}&\txt{otherwise} 
\end{cases}
\end{equation}
\end{remark}
The different steps of the NIMR method are resumed in algorithm \ref{alg:NIMR}.
\\
\begin{algorithm}[H]
\SetAlgoLined
%\underline{\textbf{\textit{Étape offline}:}}
\KwOffline{}
For $i=1,\dots,\nbrBases$, approximate the snapshots matrix $\SnapMatrix_i$ by the truncated SVD decomposition of order $\nbrModes$, that is
$$\SnapMatrix_i \approx \Mat{U}_{i} \Mat{\Sigma}_i \Mat{V}_{i}^T$$
\\
\KwOnline{}
Interpolate singular values matrices $\Mat{\Sigma}_{i}, \cdots, \Mat{\Sigma}_{i}$ and construct the matrix $\widetilde{\Mat{\Sigma}}$ associated to the untrained parameter $\widetilde{\ctrlvar}$.
\\
interpolate $[\Mat{U}_{i}]$ and $[\Mat{V}_{i}]$, $i=1,\dots,\nbrBases$ by using the ITSGM method and obtain $\widetilde{\Mat{U}}$ and $\widetilde{\Mat{V}}$ a spatial and temporal basis for the untrained parameter $\widetilde{\ctrlvar}$.
\\
Find the reference bases $\Mat{U}_{k_0}$ and $\Mat{U}_{l_0}$ and adjust signs of the sampling bases by algorithm \ref{Alg:ajust_signs_NIMR}.
\\
Calculate NIMR weights $\omega_j$ and $\kappa_j$ using equations \eqref{NIMR_spatial_weights} and \eqref{NIMR_temporal_weights}.
\\
Perform SVD decompositions 
$$\widetilde{\Mat{U}}^T \somme{i}{1}{\nbrBases} \omega_i \Mat{U}_{i} = \Mat{\xi} \Mat{\Theta} \Mat{\eta}^T
\hspace*{1cm}
\widetilde{\Mat{V}}^T \somme{i}{1}{\nbrBases} \kappa_i \Mat{U}_{i} = \Mat{\zeta} \Mat{\delta} \Mat{\gamma}^T$$
\\
Calculate $\Mat{I}_{_{\Mat{K}}}^+$ and $\Mat{I}_{_{\Mat{Q}}}^+$ and evaluate the calibration matrices $\Mat{K}$ and $\Mat{Q}$ as follows
$$\Mat{K} =  \Mat{\xi} \Mat{I}_{_{\Mat{K}}}^+ \Mat{\eta}^T
\hspace*{1cm}
\Mat{Q} =  \Mat{\zeta} \Mat{I}_{_{\Mat{Q}}}^+ \Mat{\gamma}^T$$
\\
Reconstruction of the interpolated snapshots matrix
$$\widetilde{\SnapMatrix} = \widetilde{\Mat{U}} \Mat{K} \widetilde{\Sigma} \Mat{Q}^T \widetilde{\Mat{V}}^T$$
\caption{Algorithme NIMR.}
\label{alg:NIMR}
\end{algorithm} 


==> Tex_Files/computational_cost_NIMR.tex <==
For the sake of simplicity, the approximated computational complexity of the NIMR method is detailed for the case of a one dimensional interpolation parameter ($\nbrParam = 1$) as follows
\\
\begin{itemize}
%\item \textbf{Étape 2:} interpolation of singular values is instantaneous $ \nbrBases \times  \bm{\mcal{O}} (\nbrModes)$.
\item \textbf{step 3} two ITSGM are performed for a total asymptotic cost equal to $ (3 \nbrBases-1)  \times  \left[ \bm{\mcal{O}} (\dimVecorsSnap \nbrModes^2) + \bm{\mcal{O}} (\nbrSnap \nbrModes^2) \right]$
\item \textbf{step 4} signs adjustment for a total asymptotic cost equal to $ (\nbrBases-1)  \times  \left[ \bm{\mcal{O}}(\dimVecorsSnap)  + \bm{\mcal{O}}(\nbrSnap)  + \bm{\mcal{O}}(\nbrModes^3)  \right]$
\item \textbf{Steps 5, 6 and 7:} 
\begin{itemize}
\item $2 \nbrBases$ Matrix multiplication for a total asymptotic cost equal to  $\nbrBases \times \bm{\mcal{O}} (\dimVecorsSnap \nbrModes^2) + \bm{\mcal{O}} (\nbrSnap \nbrModes^2)$.
\item two eigendecompositions for a total asymptotic cost equal to  $ 2 \bm{\mcal{O}} (\nbrModes^3) $.
\end{itemize}
\item \textbf{Step 8:} Matrix multiplication for an asymptotic cost equal to  $2 \left[  \bm{\mcal{O}} (\nbrModes^3) + \bm{\mcal{O}} (\nbrModes^2) \right] $.
\end{itemize}
\vspace*{1cm}
The total computational cost of the NIMR method for the assumed case of a one dimensional interpolation parameter grows approximately as $ 6 \nbrBases  \times  \bm{\mcal{O}} (\dimVecorsSnap \nbrModes^2)  $. Hence, this complexity is a linear function of the number of degrees of freedom of the underlying higher-order computational model, which makes the NIMR method computationally efficient.

